Change-point Detection by the Quantile LASSO Method

A simultaneous change-point detection and estimation in a piece-wise constant model is a common task in modern statistics. If, in addition, the whole estimation can be performed automatically, in just one single step without going through any hypothesis tests for non-identifiable models, or unwieldy classical a-posterior methods, it becomes an interesting, but also challenging idea. In this paper we introduce the estimation method based on the quantile LASSO approach. Unlike standard LASSO approaches, our method does not rely on typical assumptions usually required for the model errors, such as sub-Gaussian or Normal distribution. The proposed quantile LASSO method can effectively handle heavy-tailed random error distributions, and, in general, it offers a more complex view of the data as one can obtain any conditional quantile of the target distribution, not just the conditional mean. It is proved that under some reasonable assumptions the number of change-points is not underestimated with probability tenting to one, and, in addition, when the number of change-points is estimated correctly, the change-point estimates provided by the quantile LASSO are consistent. Numerical simulations are used to demonstrate these results and to illustrate the empirical performance robust favor of the proposed quantile LASSO method.

==> table1.tex <==
\begin{tabular}{cc|cr@{ }lr@{ }lr@{ }lr@{ }lr@{ }lc}
\multirow{2}{*}{$\boldsymbol{n}$} & \multirow{2}{*}{$\boldsymbol{\tau}$} & $\boldsymbol{\lambda_{AS}}$ & \multicolumn{2}{c}{$\boldsymbol{\lambda_{(2)}}$} & \multicolumn{4}{c}{\textbf{Model with $\boldsymbol{\lambda_{(2)}}$}} & \multicolumn{4}{c}{\textbf{Model with $\boldsymbol{\lambda_{AS}}$}} & \multicolumn{1}{c}{$\boldsymbol{|\widehat{\mathcal{A}_{n}}|}$} \\
 ~ & ~ & \scalebox{0.8}{Value} & \scalebox{0.8}{Mean} & \scalebox{0.8}{Std.Err.} & \multicolumn{2}{c}{\scalebox{1}{Est. Bias}} & \multicolumn{2}{c}{MSE} & \multicolumn{2}{c}{\scalebox{1}{Est. Bias}} & \multicolumn{2}{c}{MSE} & \multicolumn{1}{c}{\scalebox{0.8}{[M $|$ M $|$ M]}}  \\\hline\hline
\multicolumn{2}{c}{~} & \multicolumn{12}{c}{~}\\[-0.3cm]
\textbf{20} & 0.05 & 3.87 & 0.30 & \textit{(0.09)} & -0.32 & \textit{(0.41)} & 0.66 & \textit{(0.35)} & 0.49 & \textit{(0.46)} & 1.06 & \textit{(0.55)} & [0$|$0$|$0]\\
~ & 0.10 & 3.87 & 0.56 & \textit{(0.18)} & -0.02 & \textit{(0.40)} & 0.55 & \textit{(0.28)} & 0.39 & \textit{(0.39)} & 0.92 & \textit{(0.38)} & [0$|$0$|$0]\\
~ & 0.25 & 3.87 & 1.08 & \textit{(0.29)} & 0.03 & \textit{(0.33)} & 0.45 & \textit{(0.24)} & 0.20 & \textit{(0.33)} & 0.76 & \textit{(0.21)} & [0$|$0$|$0]\\
~ & 0.50 & 3.87 & 1.47 & \textit{(0.46)} & -0.01 & \textit{(0.31)} & 0.52 & \textit{(0.22)} & -0.04 & \textit{(0.30)} & 0.70 & \textit{(0.13)} & [0$|$0$|$0]\\
~ & 0.75 & 3.87 & 1.04 & \textit{(0.18)} & -0.03 & \textit{(0.32)} & 0.56 & \textit{(0.27)} & -0.21 & \textit{(0.32)} & 0.76 & \textit{(0.23)} & [0$|$0$|$0]\\
~ & 0.90 & 3.87 & 0.52 & \textit{(0.17)} & 0.07 & \textit{(0.41)} & 0.80 & \textit{(0.35)} & -0.33 & \textit{(0.40)} & 0.88 & \textit{(0.40)} & [0$|$0$|$0]\\
~ & 0.95 & 3.87 & 0.28 & \textit{(0.09)} & 0.34 & \textit{(0.44)} & 1.04 & \textit{(0.45)} & -0.40 & \textit{(0.49)} & 1.01 & \textit{(0.60)} & [0$|$0$|$0]\\
\multicolumn{2}{c}{~} & \multicolumn{12}{c}{~}\\[-0.3cm]
\textbf{100} & 0.05 & 2.15 & 1.67 & \textit{(0.57)} & 0.19 & \textit{(0.25)} & 0.45 & \textit{(0.22)} & 0.31 & \textit{(0.26)} & 0.61 & \textit{(0.27)} & [0$|$1$|$6]\\
~ & 0.10 & 2.15 & 2.63 & \textit{(0.85)} & 0.17 & \textit{(0.20)} & 0.40 & \textit{(0.17)} & 0.09 & \textit{(0.19)} & 0.31 & \textit{(0.14)} & [1$|$3$|$10]\\
~ & 0.25 & 2.15 & 4.73 & \textit{(1.31)} & 0.10 & \textit{(0.15)} & 0.35 & \textit{(0.13)} & 0.00 & \textit{(0.14)} & 0.14 & \textit{(0.07)} & [1$|$6$|$15]\\
~ & 0.50 & 2.15 & 6.22 & \textit{(1.51)} & -0.01 & \textit{(0.14)} & 0.41 & \textit{(0.15)} & -0.01 & \textit{(0.13)} & 0.12 & \textit{(0.06)} & [2$|$9$|$21]\\
~ & 0.75 & 2.15 & 4.40 & \textit{(0.91)} & -0.12 & \textit{(0.16)} & 0.44 & \textit{(0.18)} & 0.00 & \textit{(0.14)} & 0.16 & \textit{(0.09)} & [1$|$6$|$15]\\
~ & 0.90 & 2.15 & 2.29 & \textit{(0.45)} & -0.19 & \textit{(0.19)} & 0.56 & \textit{(0.19)} & -0.17 & \textit{(0.19)} & 0.53 & \textit{(0.18)} & [0$|$3$|$9]\\
~ & 0.95 & 2.15 & 1.36 & \textit{(0.27)} & -0.20 & \textit{(0.22)} & 0.64 & \textit{(0.20)} & -0.37 & \textit{(0.22)} & 0.80 & \textit{(0.18)} & [0$|$0$|$3]\\
\multicolumn{2}{c}{~} & \multicolumn{12}{c}{~}\\[-0.3cm]
\textbf{500} & 0.05 & 1.11 & 7.73 & \textit{(2.51)} & 0.24 & \textit{(0.13)} & 0.41 & \textit{(0.15)} & -0.06 & \textit{(0.09)} & 0.10 & \textit{(0.03)} & [7$|$15$|$25]\\
~ & 0.10 & 1.11 & 12.82 & \textit{(4.44)} & 0.19 & \textit{(0.10)} & 0.36 & \textit{(0.13)} & -0.06 & \textit{(0.07)} & 0.09 & \textit{(0.03)} & [15$|$24$|$41]\\
~ & 0.25 & 1.11 & 22.60 & \textit{(6.33)} & 0.10 & \textit{(0.07)} & 0.33 & \textit{(0.11)} & -0.04 & \textit{(0.06)} & 0.10 & \textit{(0.02)} & [37$|$53$|$69]\\
~ & 0.50 & 1.11 & 30.23 & \textit{(6.61)} & -0.01 & \textit{(0.06)} & 0.38 & \textit{(0.13)} & 0.00 & \textit{(0.05)} & 0.09 & \textit{(0.02)} & [55$|$79$|$103]\\
~ & 0.75 & 1.11 & 20.26 & \textit{(3.35)} & -0.13 & \textit{(0.08)} & 0.41 & \textit{(0.15)} & 0.04 & \textit{(0.06)} & 0.10 & \textit{(0.02)} & [38$|$53$|$71]\\
~ & 0.90 & 1.11 & 9.95 & \textit{(1.07)} & -0.23 & \textit{(0.10)} & 0.52 & \textit{(0.17)} & 0.06 & \textit{(0.08)} & 0.09 & \textit{(0.03)} & [14$|$24$|$40]\\
~ & 0.95 & 1.11 & 5.52 & \textit{(0.79)} & -0.27 & \textit{(0.13)} & 0.58 & \textit{(0.18)} & 0.06 & \textit{(0.09)} & 0.10 & \textit{(0.04)} & [6$|$15$|$27]\\
\multicolumn{2}{c}{~} & \multicolumn{12}{c}{~}\\[-0.3cm]
\hline\hline\end{tabular}


==> table2.tex <==
\begin{tabular}{ccc|r<{\hspace{-\tabcolsep}}>{\hspace{-\tabcolsep}\,}lr<{\hspace{-\tabcolsep}}>{\hspace{-\tabcolsep}\,}lr<{\hspace{-\tabcolsep}}>{\hspace{-\tabcolsep}\,}l
    r<{\hspace{-\tabcolsep}}>{\hspace{-\tabcolsep}\,}lr<{\hspace{-\tabcolsep}}>{\hspace{-\tabcolsep}\,}lr<{\hspace{-\tabcolsep}}>{\hspace{-\tabcolsep}\,}l}
\multirow{2}{*}{$\boldsymbol{\mathcal{D}}$} & & \multirow{2}{*}{$\boldsymbol{n}$} & 
     \multicolumn{4}{c}{\textbf{Model with $\boldsymbol{\lambda_{(2)}}$}} & \multicolumn{4}{c}{\textbf{Model with $\boldsymbol{\lambda_{AS}}$}} & \multicolumn{4}{c}{\textbf{Model w. $\boldsymbol{\lambda_{MS}} /$  SMUCE}} \\
 ~ & ~ & ~ & 
     \multicolumn{2}{c}{\scalebox{1}{Est. Bias}} & \multicolumn{2}{c}{MSE} & \multicolumn{2}{c}{\scalebox{1}{Est. Bias}} & \multicolumn{2}{c}{MSE} & \multicolumn{2}{c}{\scalebox{1}{Est. Bias}} & \multicolumn{2}{c}{MSE}  \\\hline\hline
\multicolumn{3}{c}{~} & \multicolumn{12}{c}{~}\\[-0.3cm]
$\boldsymbol{N}$ & \multirow{3}{*}{\rotatebox{90}{SLasso}} & \textbf{20} & 0.00 & \textit{(0.23)} & 0.43 & \textit{(0.16)} & 0.00 & \textit{(0.23)} & 0.65 & \textit{(0.08)} & 0.00 & \textit{(0.23)} & 0.27 & \textit{(0.15)} \\
 & & \textbf{100} & 0.00 & \textit{(0.10)} & 0.35 & \textit{(0.12)} & 0.00 & \textit{(0.10)} & 0.09 & \textit{(0.04)} & 0.00 & \textit{(0.10)} & 0.13 & \textit{(0.08)} \\
 & & \textbf{500} & 0.00 & \textit{(0.04)} & 0.33 & \textit{(0.11)} & 0.00 & \textit{(0.04)} & 0.06 & \textit{(0.02)} & 0.00 & \textit{(0.04)} & 0.02 & \textit{(0.01)} \\
\multicolumn{3}{c}{~} & \multicolumn{12}{c}{~}\\[-0.4cm]
\rowcolor{Gray} &  & \textbf{20} & -0.01 & \textit{(0.31)} & 0.53 & \textit{(0.21)} & -0.04 & \textit{(0.29)} & 0.70 & \textit{(0.13)} & 0.00 & \textit{(0.24)} & 0.31 & \textit{(0.17)} \\
\rowcolor{Gray} & & \textbf{100} & -0.01 & \textit{(0.14)} & 0.43 & \textit{(0.14)} & 0.00 & \textit{(0.13)} & 0.12 & \textit{(0.06)} & 0.00 & \textit{(0.13)} & 0.20 & \textit{(0.11)} \\
\rowcolor{Gray} & \multirow{-3}{*}{\rotatebox{90}{QLasso}} & \textbf{500} & -0.01 & \textit{(0.06)} & 0.40 & \textit{(0.12)} & 0.00 & \textit{(0.05)} & 0.09 & \textit{(0.02)} & 0.00 & \textit{(0.05)} & 0.03 & \textit{(0.01)} \\
\multicolumn{3}{c}{~} & \multicolumn{12}{c}{~}\\[-0.4cm]
 & \multirow{3}{*}{\rotatebox{90}{SMUCE}} & \textbf{20} &  ~  & \textit{~} & ~ & \textit{~} &  ~ & \textit{~} & ~ & \textit{~} & -0.01 & \textit{(0.23)} & 0.55 & \textit{(0.21)} \\
 & & \textbf{100} &  ~  & \textit{~} & ~ & \textit{~} &  ~ & \textit{~} & ~ & \textit{~} & 0.01 & \textit{(0.10)} & 0.12 & \textit{(0.10)} \\
 & & \textbf{500} &  ~  & \textit{~} & ~ & \textit{~} &  ~ & \textit{~} & ~ & \textit{~} & 0.00 & \textit{(0.04)} & 0.02 & \textit{(0.01)} \\
\multicolumn{3}{c}{~} & \multicolumn{12}{c}{~}\\[-0.2cm]
$\boldsymbol{t_3}$ & \multirow{3}{*}{\rotatebox{90}{SLasso}} & \textbf{20} & 0.00 & \textit{(0.38)} & 0.61 & \textit{(0.46)} & 0.00 & \textit{(0.38)} & 0.73 & \textit{(0.36)} & 0.00 & \textit{(0.38)} & 0.47 & \textit{(0.31)} \\
 & & \textbf{100} & 0.00 & \textit{(0.17)} & 0.41 & \textit{(0.14)} & 0.00 & \textit{(0.17)} & 0.33 & \textit{(0.81)} & 0.00 & \textit{(0.17)} & 0.20 & \textit{(0.11)} \\
 & & \textbf{500} & 0.00 & \textit{(0.08)} & 0.36 & \textit{(0.11)} & 0.00 & \textit{(0.08)} & 0.69 & \textit{(2.32)} & 0.00 & \textit{(0.08)} & 0.05 & \textit{(0.03)} \\
\multicolumn{3}{c}{~} & \multicolumn{12}{c}{~}\\[-0.4cm]
\rowcolor{Gray} &  & \textbf{20} & -0.01 & \textit{(0.35)} & 0.59 & \textit{(0.28)} & -0.04 & \textit{(0.34)} & 0.73 & \textit{(0.16)} & 0.01 & \textit{(0.28)} & 0.39 & \textit{(0.21)} \\
\rowcolor{Gray} & & \textbf{100} & -0.01 & \textit{(0.15)} & 0.44 & \textit{(0.14)} & 0.00 & \textit{(0.14)} & 0.15 & \textit{(0.08)} & 0.00 & \textit{(0.14)} & 0.24 & \textit{(0.12)} \\
\rowcolor{Gray} & \multirow{-3}{*}{\rotatebox{90}{QLasso}} & \textbf{500} & -0.02 & \textit{(0.07)} & 0.42 & \textit{(0.13)} & 0.00 & \textit{(0.06)} & 0.11 & \textit{(0.03)} & 0.00 & \textit{(0.06)} & 0.04 & \textit{(0.02)} \\
\multicolumn{3}{c}{~} & \multicolumn{12}{c}{~}\\[-0.4cm]
 & \multirow{3}{*}{\rotatebox{90}{SMUCE}} & \textbf{20} &  ~  & \textit{~} & ~ & \textit{~} &  ~ & \textit{~} & ~ & \textit{~} & -0.01 & \textit{(0.39)} & 1.33 & \textit{(2.06)} \\
 & & \textbf{100} &  ~  & \textit{~} & ~ & \textit{~} &  ~ & \textit{~} & ~ & \textit{~} & 0.01 & \textit{(0.19)} & 1.08 & \textit{(1.60)} \\
 & & \textbf{500} &  ~  & \textit{~} & ~ & \textit{~} &  ~ & \textit{~} & ~ & \textit{~} & 0.00 & \textit{(0.09)} & 0.95 & \textit{(2.52)} \\
\multicolumn{3}{c}{~} & \multicolumn{12}{c}{~}\\[-0.2cm]
$\boldsymbol{C}$ & \multirow{3}{*}{\rotatebox{90}{SLasso}} & \textbf{20} & -1.57 & \textit{(74.19)} & 5867 & \textit{(154600)} & -1.57 & \textit{(74.19)} & 109736 & \textit{(3089261)} & -1.57 & \textit{(74.19)} & 5785 & \textit{(154589)} \\
 & & \textbf{100} & -1.15 & \textit{(22.21)} & 524 & \textit{(7333)} & -1.15 & \textit{(22.21)} & 50589 & \textit{(765657)} & -1.15 & \textit{(22.21)} & 512 & \textit{(7322)} \\
 & & \textbf{500} & -1.65 & \textit{(36.73)} & 1354 & \textit{(24483)} & -1.65 & \textit{(36.72)} & 671194 & \textit{(12245127)} & -1.65 & \textit{(36.72)} & 1353 & \textit{(24477)} \\
\multicolumn{3}{c}{~} & \multicolumn{12}{c}{~}\\[-0.4cm]
\rowcolor{Gray} &  & \textbf{20} & -0.02 & \textit{(0.46)} & 0.75 & \textit{(0.48)} & -0.03 & \textit{(0.44)} & 0.81 & \textit{(0.30)} & 0.01 & \textit{(0.36)} & 0.53 & \textit{(0.30)} \\
\rowcolor{Gray} & & \textbf{100} & -0.02 & \textit{(0.20)} & 0.49 & \textit{(0.16)} & -0.02 & \textit{(0.18)} & 0.20 & \textit{(0.12)} & -0.01 & \textit{(0.18)} & 0.28 & \textit{(0.15)} \\
\rowcolor{Gray} & \multirow{-3}{*}{\rotatebox{90}{QLasso}} & \textbf{500} & -0.02 & \textit{(0.09)} & 0.44 & \textit{(0.14)} & 0.00 & \textit{(0.08)} & 0.18 & \textit{(0.06)} & 0.00 & \textit{(0.07)} & 0.05 & \textit{(0.03)} \\
\multicolumn{3}{c}{~} & \multicolumn{12}{c}{~}\\[-0.4cm]
 & \multirow{3}{*}{\rotatebox{90}{SMUCE}} & \textbf{20} &  ~  & \textit{~} & ~ & \textit{~} &  ~ & \textit{~} & ~ & \textit{~} & -1.58 & \textit{(74.19)} & 109953 & \textit{(3091453)} \\
 & & \textbf{100} &  ~  & \textit{~} & ~ & \textit{~} &  ~ & \textit{~} & ~ & \textit{~} & -1.16 & \textit{(22.21)} & 50683 & \textit{(766016)} \\
 & & \textbf{500} &  ~  & \textit{~} & ~ & \textit{~} &  ~ & \textit{~} & ~ & \textit{~} & -1.65 & \textit{(36.72)} & 671259 & \textit{(12245434)} \\
\multicolumn{3}{c}{~} & \multicolumn{12}{c}{~}\\[-0.2cm]
\hline\hline\end{tabular}


==> table3.tex <==
\begin{tabular}{ccc|cccccr<{\hspace{-\tabcolsep}}>{\hspace{-\tabcolsep}\,}lr<{\hspace{-\tabcolsep}}>{\hspace{-\tabcolsep}\,}lc<{\hspace{-\tabcolsep}}>{\hspace{-\tabcolsep}\,}l}
\multirow{2}{*}{$\boldsymbol{\mathcal{D}}$} & & \multirow{2}{*}{$\boldsymbol{n}$} & 
    $\boldsymbol{\lambda_{AS}}$ & \multicolumn{1}{c}{$\boldsymbol{\lambda_{(2)}}$} & \multicolumn{1}{c}{$\boldsymbol{\lambda_{MS}}$} & \multicolumn{2}{c}{Number of Jumps $\boldsymbol{|\widehat{\cal A}_n|}$} & 
      \multicolumn{6}{c}{\textbf{Change-point Detection Error}} \\
 ~ & ~ & ~ & Value & Avg. & Avg. & $\lambda_{AS}$ & $\lambda_{MS}$/\scalebox{0.8}{SMUCE} & \multicolumn{2}{c}{(with $\lambda_{(2)}$)} & \multicolumn{2}{c}{(with $\lambda_{AS}$)} & \multicolumn{2}{c}{($\lambda_{CV}$/\scalebox{0.8}{SMUCE})} \\\hline\hline
\multicolumn{3}{c}{~} & \multicolumn{11}{c}{~}\\[-0.3cm]
$\boldsymbol{N}$ & \multirow{3}{*}{\rotatebox{90}{SLasso}} & \textbf{20} & 3.87 & 1.68 & 0.98 & [0$|$0$|$3] & [0$|$0$|$11] & 0.08 & \textit{(0.06)} & 0.17 & \textit{(0.03)} & 0.04 & \textit{(0.04)} \\
  &  & \textbf{100} & 2.15 & 7.77 & 3.29 & [2$|$2$|$14] & [2$|$2$|$21] & 0.02 & \textit{(0.02)} & 0.01 & \textit{(0.01)} & 0.01 & \textit{(0.01)} \\
  &  & \textbf{500} & 1.11 & 38.09 & 4.54 & [32$|$32$|$66] & [3$|$3$|$23] & 0.00 & \textit{(0.00)} & 0.00 & \textit{(0.00)} & 0.00 & \textit{(0.00)} \\
\multicolumn{3}{c}{~} & \multicolumn{11}{c}{~}\\[-0.4cm]
\rowcolor{Gray} & ~ & \textbf{20} & 3.87 & 1.58 & 1.17 & [0$|$0$|$0] & [0$|$0$|$13] & 0.10 & \textit{(0.07)} & NaN & \textit{(NA)} & 0.04 & \textit{(0.04)} \\
\rowcolor{Gray}  &  & \textbf{100} & 2.15 & 6.54 & 4.00 & [2$|$2$|$21] & [1$|$1$|$28] & 0.03 & \textit{(0.04)} & 0.01 & \textit{(0.01)} & 0.01 & \textit{(0.03)} \\
\rowcolor{Gray}  & \multirow{-3}{*}{\rotatebox{90}{QLasso}} & \textbf{500} & 1.11 & 31.31 & 4.68 & [35$|$35$|$70] & [4$|$4$|$65] & 0.00 & \textit{(0.00)} & 0.00 & \textit{(0.00)} & 0.00 & \textit{(0.00)} \\
\multicolumn{3}{c}{~} & \multicolumn{11}{c}{~}\\[-0.4cm]
 & \multirow{3}{*}{\rotatebox{90}{SMUCE}} & \textbf{20} &  ~ & ~ & ~ &  ~ & [0$|$0$|$4] &  ~ & ~ &  ~ & ~ & 0.07 & \textit{(0.04)} \\
  &  & \textbf{100} &  ~ & ~ & ~ &  ~ & [0$|$1$|$4] &  ~ & ~ &  ~ & ~ & 0.02 & \textit{(0.03)} \\
  &  & \textbf{500} &  ~ & ~ & ~ &  ~ & [2$|$2$|$3] &  ~ & ~ &  ~ & ~ & 0.00 & \textit{(0.00)} \\
\multicolumn{3}{c}{~} & \multicolumn{11}{c}{~}\\[-0.2cm]
$\boldsymbol{t_3}$ & \multirow{3}{*}{\rotatebox{90}{SLasso}} & \textbf{20} & 3.87 & 2.14 & 2.25 & [0$|$0$|$5] & [0$|$0$|$9] & 0.10 & \textit{(0.06)} & 0.12 & \textit{(0.06)} & 0.06 & \textit{(0.05)} \\
  &  & \textbf{100} & 2.15 & 8.86 & 4.02 & [3$|$3$|$23] & [1$|$1$|$14] & 0.05 & \textit{(0.05)} & 0.02 & \textit{(0.02)} & 0.02 & \textit{(0.03)} \\
  &  & \textbf{500} & 1.11 & 41.10 & 7.61 & [67$|$67$|$124] & [3$|$3$|$23] & 0.01 & \textit{(0.02)} & 0.00 & \textit{(0.00)} & 0.00 & \textit{(0.00)} \\
\multicolumn{3}{c}{~} & \multicolumn{11}{c}{~}\\[-0.4cm]
\rowcolor{Gray} & ~ & \textbf{20} & 3.87 & 1.52 & 1.55 & [0$|$0$|$0] & [0$|$0$|$13] & 0.11 & \textit{(0.06)} & NaN & \textit{(NA)} & 0.05 & \textit{(0.05)} \\
\rowcolor{Gray}  &  & \textbf{100} & 2.15 & 6.03 & 3.91 & [2$|$2$|$20] & [0$|$0$|$26] & 0.04 & \textit{(0.05)} & 0.01 & \textit{(0.02)} & 0.02 & \textit{(0.04)} \\
\rowcolor{Gray}  & \multirow{-3}{*}{\rotatebox{90}{QLasso}} & \textbf{500} & 1.11 & 28.98 & 4.59 & [54$|$54$|$104] & [4$|$4$|$36] & 0.01 & \textit{(0.01)} & 0.00 & \textit{(0.00)} & 0.00 & \textit{(0.00)} \\
\multicolumn{3}{c}{~} & \multicolumn{11}{c}{~}\\[-0.4cm]
 & \multirow{3}{*}{\rotatebox{90}{SMUCE}} & \textbf{20} &  ~ & ~ & ~ &  ~ & [0$|$0$|$6] &  ~ & ~ &  ~ & ~ & 0.09 & \textit{(0.05)} \\
  &  & \textbf{100} &  ~ & ~ & ~ &  ~ & [0$|$2$|$10] &  ~ & ~ &  ~ & ~ & 0.05 & \textit{(0.05)} \\
  &  & \textbf{500} &  ~ & ~ & ~ &  ~ & [2$|$2$|$23] &  ~ & ~ &  ~ & ~ & 0.02 & \textit{(0.02)} \\
\multicolumn{3}{c}{~} & \multicolumn{11}{c}{~}\\[-0.2cm]
$\boldsymbol{C}$ & \multirow{3}{*}{\rotatebox{90}{SLasso}} & \textbf{20} & 3.87 & 112.40 & 83.71 & [0$|$0$|$17] & [0$|$1$|$19] & 0.12 & \textit{(0.06)} & 0.08 & \textit{(0.06)} & 0.10 & \textit{(0.06)} \\
  &  & \textbf{100} & 2.15 & 386.53 & 237.47 & [7$|$7$|$96] & [0$|$0$|$96] & 0.12 & \textit{(0.06)} & 0.01 & \textit{(0.01)} & 0.07 & \textit{(0.06)} \\
  &  & \textbf{500} & 1.11 & 1414.77 & 1353.09 & [164$|$164$|$493] & [0$|$0$|$499] & 0.10 & \textit{(0.06)} & 0.00 & \textit{(0.00)} & 0.08 & \textit{(0.06)} \\
\multicolumn{3}{c}{~} & \multicolumn{11}{c}{~}\\[-0.4cm]
\rowcolor{Gray} & ~ & \textbf{20} & 3.87 & 1.45 & 2.66 & [0$|$0$|$1] & [0$|$0$|$12] & 0.12 & \textit{(0.06)} & 0.07 & \textit{(NA)} & 0.06 & \textit{(0.05)} \\
\rowcolor{Gray}  &  & \textbf{100} & 2.15 & 5.27 & 3.65 & [2$|$2$|$22] & [0$|$0$|$39] & 0.05 & \textit{(0.05)} & 0.02 & \textit{(0.02)} & 0.03 & \textit{(0.04)} \\
\rowcolor{Gray}  & \multirow{-3}{*}{\rotatebox{90}{QLasso}} & \textbf{500} & 1.11 & 24.58 & 4.86 & [54$|$54$|$192] & [2$|$2$|$42] & 0.01 & \textit{(0.01)} & 0.00 & \textit{(0.00)} & 0.00 & \textit{(0.00)} \\
\multicolumn{3}{c}{~} & \multicolumn{11}{c}{~}\\[-0.4cm]
 & \multirow{3}{*}{\rotatebox{90}{SMUCE}} & \textbf{20} &  ~ & ~ & ~ &  ~ & [0$|$0$|$7] &  ~ & ~ &  ~ & ~ & 0.10 & \textit{(0.05)} \\
  &  & \textbf{100} &  ~ & ~ & ~ &  ~ & [1$|$1$|$22] &  ~ & ~ &  ~ & ~ & 0.05 & \textit{(0.04)} \\
  &  & \textbf{500} &  ~ & ~ & ~ &  ~ & [25$|$25$|$72] &  ~ & ~ &  ~ & ~ & 0.01 & \textit{(0.01)} \\
\multicolumn{3}{c}{~} & \multicolumn{11}{c}{~}\\[-0.2cm]
\hline\hline\end{tabular}

